Inpainting at Modern Camera Resolution by Guided PatchMatch with Auto-Curation

Recently, deep models have established SOTA performance for low-resolution image inpainting, but they lack fidelity at resolutions associated with modern cameras such as 4K or more, and for large holes. We contribute an inpainting benchmark dataset of photos at 4K and above representative of modern sensors. We demonstrate a novel framework that combines deep learning and traditional methods. We use an existing deep inpainting model LaMa to fill the hole plausibly, establish three guide images consisting of structure, segmentation, depth, and apply a multiply-guided PatchMatch to produce eight candidate upsampled inpainted images. Next, we feed all candidate inpaintings through a novel curation module that chooses a good inpainting by column summation on an 8x8 antisymmetric pairwise preference matrix. Our framework's results are overwhelmingly preferred by users over 8 strong baselines, with improvements of quantitative metrics up to 7.4 over the best baseline LaMa, and our technique when paired with 4 different SOTA inpainting backbones improves each such that ours is overwhelmingly preferred by users over a strong super-res baseline.

==> figs/auto_manual_selection.tex <==
\begin{figure*}[!t]
    \centering
    %[trim=left bottom right top,
    \includegraphics[trim=0.6in 2.4in 0.4in 0.0in, clip,width=7in]{auto_manual_selection.pdf}
    \caption{This figure illustrates an example of user selection and network selection on 8 guided PatchMatch outputs. The top 3 user selections are indicated by the green bounding boxes, where the preference order is indicated by the shade of green (from dark green to light green). The network selected result is indicated by the red bounding box. In this case, our network selection aligns with the top 1 user preference. }
    \label{fig:auto_manual_selection}
\end{figure*}






==> figs/auto_selection_new.tex <==
\begin{figure*}[!t]
    \centering
    %[trim=left bottom right top,
    \includegraphics[trim=0.0in 1.0in 0.0in 1.0in, clip,width=7in]{auto_selection_new.pdf}
    \caption{Qualitative comparison of automatic selection results for Guided PatchMatch using our trained selection network. The titles at the top represent the guide types for PatchMatch. The {\color{red} red bounding box} around images in each row indicates the selected image among the eight candidates. Please feel free to zoom-in to check the details.}
    \label{fig:auto_selection_new}
\end{figure*}






==> figs/cam_vis.tex <==
\begin{figure}[h]
    \centering
    %[trim=left bottom right top,
    \includegraphics[trim=3.6in 0.8in 3.4in 0.0in, clip,width=3.35in]{cam_vis.pdf}
    \caption{Grad-CAM [Selvaraju et al.] visualization of our selection network on three guided PatchMatch outputs.  More descriptions can be found in section \ref{sec:visualizations}.}
    \label{fig:cam_vis}
\end{figure}





==> figs/comparison_with_sota.tex <==
\begin{figure*}[t]
    \centering
    %[trim=left bottom right top,
    \includegraphics[width=7in]{comparison_with_sota_v2.pdf}
    \caption{Qualitative comparison with state-of-the-art image inpainting methods. Please zoom in and observe that ours has significantly more texture detail than previous work run in the ``local crop" setup that we found was best from our comparisons and user study. Our results are either good enough to use as a high-quality print result or could be improved with only minor retouching.}
    \label{fig:comparison_with_sota}
\end{figure*}


==> figs/limitations.tex <==
\begin{figure*}[h]
    \centering
    %[trim=left bottom right top,
    \includegraphics[width=7in]{limitations.pdf}
    \caption{Limitations of our method and ways they can be mitigated through user interactions. In (a), regular structures under perspective can be broken. In (b), the segmentation map within a human is too coarse grained, so clothing and skin are not distinguished. Even without this information, a manually selected result (c) using a structure map is somewhat better. In (d), there is not yet a reliable instance segmentation for penguins. In the meantime, the user can manually brush to improve the depth and segmentation map and obtain a better result. In (f) we see that geometric transformations of patches would be needed. Even without this, however, a user can manually pick a result (g) (with no guides) that has slightly better line continuity.}
    \label{fig:limitations}
\end{figure*}

==> figs/manual_selection.tex <==
\begin{figure*}[!t]
    \centering
    %[trim=left bottom right top,
    \includegraphics[trim=0.0in 2.6in 0.0in 0.0in, clip,width=7in]{manual_selection.pdf}
    \caption{Qualitative comparison of manual selection by an oracle (user study). The {\color{blue} blue bounding boxes} around images in each row indicates the top three user selected image among the eight candidates. Please feel free to zoom-in to check the details. \Lingzhi{Merge with next figure, leave two input images that have great results and user study choices are reasonable, and make input image and results bigger by putting results on two rows.}}
    \label{fig:manual_selection}
\end{figure*}






==> figs/multi_source_guide.tex <==
\begin{figure*}[h]
    \centering
    %[trim=left bottom right top,
    \includegraphics[trim=2.0in 0.7in 2.0in 0in, clip,width=7in]{multi_source_guide.pdf}
    \caption{Qualitative comparison between Single-source guided PatchMatch and Multi-source guided PatchMatch. The input images are shown in the first column. Two single-source guided PatchMatch outputs are shown in the second and third columns, and the multi-source guided PatchMatch outputs are in the last column. The guide images (depth, structure, segmentation) used in each case are shown in the top left corner of the output images. }
    \label{fig:multi_source_guide}
\end{figure*}






==> figs/single_source_guide.tex <==
\begin{figure}
    \centering
    %[trim=left bottom right top,
    \includegraphics[trim=2.4in 0.0in 3.0in 0in, clip,width=3.4in]{single_source_guide.pdf}
    \caption{PatchMatch guided by only a single guide. In the second column, we show the selected guided PatchMatch output from our network, and the used guide is shown in the top right corner. Please zoom to see details.}
    \label{fig:single_source_guide}
\end{figure}




==> tables/guided_patchmatch.tex <==
\begin{table*}[h!]
    \begin{center}
      \begin{tabular}{l|c|c|c|c|c}
        \toprule % <-- Toprule here
        \textbf{Methods} & \textbf{BG20K} \cite{li2020end} & \textbf{DIV2K} \cite{Ignatov_2018_ECCV_Workshops} & \textbf{DIV8K} \cite{gu2019div8k} & \textbf{User Photos} & \textbf{Overall} \\
        \midrule % <-- Midrule here
        No Guide & 23.00\% & 26.00\% & 24.50\% & 21.00\% & 23.63\% \\
        Depth & 33.50\% & 39.00\% & 36.00\% & 34.50\% & 35.00\% \\
        Structure & 39.00\% & 34.00\% & 29.50\% & 40.00\% & 35.63\% \\
        Segmentation & 30.50\% & 33.50\% & 27.50\% & 38.50\% & 32.50\% \\
        Depth + Seg & 46.00\% & 40.00\% & 40.00\% & 43.50\% & 42.38\% \\
        Depth + Struct & 45.00\% & 43.50\% & 47.00\% & 42.00\% & 44.38\% \\
        Struct + Seg & 51.50\% & 47.50\% & 49.50\% & 52.00\% & 50.13\% \\
        Depth + Struct + Seg & 31.50\% & 36.50\% & 46.00\% & 31.50\% & 36.38\% \\
        \midrule
        SelectionNet w/o mask & 55.00\% & 51.00\% & 55.00\% & 53.50\% & 53.63\% \\
        SelectionNet w/ mask & 55.50\% & 53.00\% & 57.00\% & 55.50\% & 55.25\% \\
        \bottomrule % <-- Bottomrule here
      \end{tabular}
      \vspace{5 pt}
      \caption{Quantitative user preferences for guided PatchMatch variants. In this user study, we ask each user to select top 3 best images among the eight candidates. The table above shows the chance that each type of guided PatchMatch is selected by users in terms of percentage. The user study is conducted on Amazon Mechanical Turk (AMT). We consider the bottom row (selection with mask) to be our full method.}
      \label{tab:different_guides}
    \end{center}
\end{table*}




==> tables/improve_4_deep_models.tex <==
\begin{table}[h!]
    \begin{center}
     \resizebox{0.6\textwidth}{!}{
      \begin{tabular}{l|c|c|c}
        \toprule % <-- Toprule here
        \textbf{Methods} & \textbf{LPIPS $\downarrow$} & \textbf{FID $\downarrow$} & \textbf{User Pref. $\uparrow$} \\
        \midrule % <-- Midrule here
        ProFill \cite{zeng2020high} + SR \cite{wang2021real} & 0.0478 & 24.2589 & 21 \\
        ProFill \cite{zeng2020high} + Ours & \textbf{0.0425} & \textbf{20.4362} & \textbf{179}  \\
        \midrule
        CoModGAN \cite{zhao2021comodgan} + SR \cite{wang2021real} & 0.0510 & 24.8189 & 36 \\
        CoModGAN \cite{zhao2021comodgan} + Ours & \textbf{0.0430} & \textbf{19.9224} & \textbf{164}  \\ 
        \midrule % <-- Midrule here
        MADF \cite{zhu2021image} + SR \cite{wang2021real} & 0.0477 & 23.6290 & 27 \\
        MADF \cite{zhu2021image} + Ours & \textbf{0.0421} & \textbf{19.9022} & \textbf{173}  \\
        \midrule
        LaMa \cite{suvorov2021resolution} + SR \cite{wang2021real} & 0.04588 & 19.2022 & 42 \\
        LaMa \cite{suvorov2021resolution} + Ours & \textbf{0.04156} & \textbf{18.7414} & \textbf{158} \\
        \bottomrule % <-- Bottomrule here
      \end{tabular}
      }
    %   \vspace{5 pt}
      \caption{A pairwise comparison study between high-resolution inpainting results for upsampled by Real-ESRGAN \cite{wang2021real} and results upsampled by our framework, for four recent inpainting methods \cite{zeng2020high,zhao2021comodgan,zhu2021image,suvorov2021resolution}. We show similar results for 3 older inpainting models in the supplemental. The users are asked to choose the best image from a pair of images for each type of inpainting model. The best score in each case are bold text.  }
      \label{tab:improve_4_deep_models}
    \end{center}
    \vspace{-15 pt}
\end{table}







==> tables/pm_random_ours.tex <==
\begin{table}[h!]
    \begin{center}
      \begin{tabular}{l|c|c|c}
        \toprule % <-- Toprule here
        \textbf{Methods} & \textbf{LPIPS $\downarrow$} & \textbf{FID $\downarrow$} & \textbf{User Pref. $\uparrow$} \\
        \midrule % <-- Midrule here
        Content-Aware Fill & 0.04675 & 23.0068 & 16 \\
        Random Guided PM & 0.04281 & 19.7704 & 24 \\
        SuperCAF (Ours) & \textbf{0.04156} & \textbf{18.7414} & \textbf{60} \\
        \bottomrule % <-- Bottomrule here
      \end{tabular}
    %   \vspace{5 pt}
      \caption{A comparison study with Photoshop's Content-Aware Fill, which is based on PatchMatch~\cite{barnes2009patchmatch} and a randomly selected Guided PatchMatch baseline. Photos average 20 megapixels and holes average 2.3 megapixels. The user studies are performed on 100 photographs where all method outputs are different from each other. The best scores are bold text in the table.}
      \label{tab:pm_random_ours}
    \end{center}
    \vspace{-20 pt}
\end{table}



